SpreadsheetBench: Towards Challenging Real World Spreadsheet Manipulation

We introduce SpreadsheetBench, a challenging spreadsheet manipulation benchmark exclusively derived from real-world scenarios, designed to immerse current large language models (LLMs) in the actual workflow of spreadsheet users. Unlike existing benchmarks that rely on synthesized queries and simplified spreadsheet files, SpreadsheetBench is built from 912 real questions gathered from online Excel forums, which reflect the intricate needs of users. The associated spreadsheets from the forums contain a variety of tabular data such as multiple tables, non-standard relational tables, and abundant non-textual elements. Furthermore, we propose a more reliable evaluation metric akin to online judge platforms, where multiple spreadsheet files are created as test cases for each instruction, ensuring the evaluation of robust solutions capable of handling spreadsheets with varying values. Our comprehensive evaluation of various LLMs under both single-round and multi-round inference settings reveals a substantial gap between the state-of-the-art (SOTA) models and human performance, highlighting the benchmark's difficulty.

==> latex/4.related_work.tex <==
% There exist some benchmarks target spreadsheet manipulation.
% SheetCopilot and InstructExcel focus on the breadth of spreadsheet operations, covering 44 operations that are categorized as \textit{Entry \& manipulation}, \textit{Management}, etc.
% SheetRM formulize the spreadsheet manipulation task as a multi-step reasoning process which involve more than one spreadsheet operations.
% involve multi-step reasoning process by combining multiple types of spreadsheet manipulations to a single query.
% combine the atomic manipulations to evaluate the reasoning ability of spreadsheet agent.

\textbf{Table-related Dataset.}
Traditional table-related datasets focus on table question answering~\cite{pasupat2015wtq} and table-to-text generation tasks~\cite{parikh2020totto}.
Table question answering (TableQA) requires models to answer questions based on the content or the description of tables~\cite{zhu2021tat-qa, chen2021ottqa, cheng2022hitab}.
Table-to-text generation requires models to generate a description from the structured table~\cite{zhao2023loft, zhao2023investigating}.
Recently, researchers show interest in data analysis~\cite{hu2024infiagent} and spreadsheet manipulation tasks~\cite{li2024sheetcopilot}.
Data analysis tasks require models to analyze tabular data and provide insights or analytical descriptions~\cite{he2024text2analysis, li2024tapilot}.
Spreadsheet manipulation tasks require LLMs to directly manipulate the spreadsheet to perform tasks such as \textit{Delete}, \textit{Insert}, etc.
SheetCopilot~\cite{li2024sheetcopilot} construct a benchmark with 221 tasks and 28 spreadsheet files, covering 44 operations that are categorized as \textit{Entry \& manipulation}, \textit{Management}, etc.
InstructExcel~\cite{payan2023instructexcel} presents a comprehensive benchmark that encompasses over 170 Excel operations across a collection of 2,000 publicly accessible Excel spreadsheets.
SheetRM~\cite{chen2024sheetagent} formulize the spreadsheet manipulation task as a multi-step reasoning process which involve more than one spreadsheet operations.
Different from existing spreadsheet manipulation benchmarks, \bench is derived purely from online forums and blogs, which is much more diverse and challenging, reflect the real-world spreadsheet manipulation scenario.

\textbf{Automatic Spreadsheet Manipulation.}
In the early years, program synthesis are used to assistant for spreadsheet manipulation~\cite{gulwani2011automating-string, gulwani2012spreadsheet-man}.
Afterwards, some researchers employ deep learning technique to automatic spreadsheet manipulation~\cite{chen2021spreadsheetcoder, chen2024auto-formula}.
Recently, benefiting from the powerful capabilities of large language models, spreadsheet agents have been developed to assist people in manipulating spreadsheets by converting natural language into specific manipulation actions.
SheetCopilot~\cite{li2024sheetcopilot} introduce an autonomous agent for  spreadsheet manipulation based on a set of atomic actions and a state machine-based task planning framework.
SheetAgent~\cite{chen2024sheetagent} creates an autonomous agent by incorporating three collaborative modules to improve the spreadsheet agent's reasoning capabilities.

